Efficient Summing over Sliding Windows

This paper considers the problem of maintaining statistic aggregates over the last W elements of a data stream. First, the problem of counting the number of 1's in the last W bits of a binary stream is considered. A lower bound of {\Omega}(1/{\epsilon} + log W) memory bits for W{\epsilon}-additive approximations is derived. This is followed by an algorithm whose memory consumption is O(1/{\epsilon} + log W) bits, indicating that the algorithm is optimal and that the bound is tight. Next, the more general problem of maintaining a sum of the last W integers, each in the range of {0,1,...,R}, is addressed. The paper shows that approximating the sum within an additive error of RW{\epsilon} can also be done using {\Theta}(1/{\epsilon} + log W) bits for {\epsilon}={\Omega}(1/W). For {\epsilon}=o(1/W), we present a succinct algorithm which uses B(1 + o(1)) bits, where B={\Theta}(Wlog(1/W{\epsilon})) is the derived lower bound. We show that all lower bounds generalize to randomized algorithms as well. All algorithms process new elements and answer queries in O(1) worst-case time.

==> basic-counting-algorithm-pseudo-code-original.tex <==
\scriptsize
\begin{algorithm}[tb]
\caption{Additive Approximation of Basic Counting}\label{alg:BasicCounting}
\scriptsize
\begin{algorithmic}[1]
\State Initialization: $y = 0, b = 0, m = 0, i=0$.
\Function{add}{Bit $x$}
\If {$m = {W\over k} - 1$}
	\State $B = B - b_i$
	\If {$y+x\geq {W\over k}$}
		\State $b_i = 1$
		\State $y = y - {W\over k} + x$
	\Else
		\State $b_i = 0$
		\State $y = y + x$
	\EndIf
	\State $B = B + b_i$
	\State $m = 0$
	\State $i = i+1 \mod k$	
\Else
	\State $y = y + x$
	\State $m = m + 1$
\EndIf
\EndFunction

\Function{Query}{}
\State \Return {${W\over k} \cdot B + y  - \frac{W}{2k}- m\cdot b_i$}
\EndFunction
\end{algorithmic}
\end{algorithm}
\normalsize

==> multiplicative-basic_counting.tex <==
\subsection{Multiplicative Approximation}

\newcommand{\epsThresh}{\frac{\log^3 \window}{\window}}
\newcommand{\timestampArraySize}{\frac{1}{\eps}\logw}
\newcommand{\timestampArraySizeSymbol}{\chi}

\newcommand{\additiveEpsilon}{\frac{\logw}{\window}}

Datar et al. provide a $1(+\eps)$-approximation that uses $O(\frac{1}{\epsilon}\log^2 \window)$ memory bits. We present an algorithm computing requiring asymptotically less memory for the case of $\eps=o(\epsThresh)$.
The algorithm uses an instance of our additive \bc{} algorithm, denoted $A$ and an array of size $\timestampArraySizeSymbol\triangleq\timestampArraySize$ which contains timestamps (each requires $\logw$ bits). When there are more than $\timestampArraySizeSymbol$ $1$'s in the window, the algorithm answers queries by returning $A$'s answer, and otherwise uses the array.

The algorithm keeps the following variables:
\begin{description}
\item[$A$] - An instance of Algorithm \ref{alg:BasicCounting} computing $\window\cdot\additiveEpsilon=\logw$-additive approximation.
\item[$o$] - the index of the current offset.
\item[$T$] - An array of size $\timestampArraySize$ containing timestamps.
\item[$V$] - A bit array of size $\timestampArraySize$ keeping whether a record in $V$ was created within the last window.
\item[$t$] - The index of the oldest entry in $T$.
\item[$\tau$] - The sum of non-expired time stamps recorded in $T$.
\end{description}

\begin{algorithm}[tb]
\caption{Multiplicative Approximation of Basic Counting}\label{alg:MultBasicCounting}
\begin{algorithmic}[1]
\State Initialization: $T=0, V=0, t=0$.
\Function{add}{Bit $x$}
\State $A.Add(x)$
\State $o = o+1 \mod \window$
\If {$x = 1$}
	\State $b_i = 1$
	\State $y = y - {W\over k} + x$
\Else
	\State $b_i = 0$
	\State $y = y + x$
\EndIf
\EndFunction

\Function{Query}{}
\State \Return {${W\over k} \cdot B + y  - \frac{W}{2k}- m\cdot b_i$}
\EndFunction
\end{algorithmic}
\end{algorithm}
